Polymorphic Coverage Types

Test input generators are an important part of property-based testing (PBT) frameworks, and a key expectation is that they be capable of producing all acceptable elements that satisfy both the function's input type and the generator-provided constraints. However, it is not readily apparent how to validate whether a particular generator's output satisfies this coverage requirement. In practice, developers typically rely on manual inspection and post-mortem analysis of test runs to determine whether a generator provides sufficient coverage; these approaches are error-prone and difficult to scale as generators grow more complex. To address this problem, we present a new refinement-type-based verification procedure for validating the coverage provided by input test generators, based on a novel interpretation of types that embeds "must-style" underapproximate reasoning principles as a fundamental part of the type system. In our formulation, the types associated with expressions capture the set of values guaranteed to be produced by the expression, rather than the usual interpretation in which types represent the set of values an expression may produce. We formalize the notion of coverage types in a rich core language supporting higher-order functions and inductive datatypes. To better support real-world test generators, we extend this type system with type and qualifier polymorphism, enabling static verification of coverage guarantees for test input generators constructed using the monadic combinators found in most PBT frameworks. Finally, we have implemented a coverage type checker for OCaml programs based on this core calculus and present a detailed evaluation of its utility using a corpus of benchmarks drawn from both the PBT literature and open-source projects.

==> Makefile <==
.PHONY: haste all clean cleanall nocite

all: poirot-jfp.pdf poirot-jfp-diff.pdf poirot-jfp-sm-full.pdf

poirot-jfp.pdf: main.tex bibliography.bib sections/intro.tex sections/motivation.tex \
	sections/languages.tex sections/rules.tex sections/algorithm.tex sections/poly.tex \
	sections/monad.tex sections/evaluation.tex sections/related.tex commands.sty
	pdflatex -jobname="poirot-jfp" -shell-escape main
	bibtex poirot-jfp
	clear
	pdflatex -jobname="poirot-jfp" -shell-escape main
	clear
	pdflatex -jobname="poirot-jfp" -shell-escape main

poirot-jfp-diff.pdf: main.tex bibliography.bib sections/intro.tex sections/motivation.tex \
	sections/languages.tex sections/rules.tex sections/algorithm.tex sections/poly.tex \
	sections/monad.tex sections/evaluation.tex sections/related.tex commands.sty
	pdflatex -jobname="poirot-jfp-diff" -shell-escape "\def\diffmode{}\input main.tex"
	bibtex poirot-jfp-diff
	clear
	pdflatex -jobname="poirot-jfp-diff" -shell-escape "\def\diffmode{}\input main.tex"
	clear
	pdflatex -jobname="poirot-jfp-diff" -shell-escape "\def\diffmode{}\input main.tex"

poirot-jfp-sm-full.pdf: main.tex bibliography.bib sections/intro.tex sections/motivation.tex \
	sections/languages.tex sections/rules.tex sections/algorithm.tex sections/poly.tex \
	sections/monad.tex sections/evaluation.tex sections/related.tex commands.sty
	pdflatex -jobname="poirot-jfp-sm-full" -shell-escape "\def\showappendix{true}\input main.tex"
	bibtex poirot-jfp-sm-full
	clear
	pdflatex -jobname="poirot-jfp-sm-full" -shell-escape "\def\showappendix{true}\input main.tex"
	clear
	pdflatex -jobname="poirot-jfp-sm-full" -shell-escape "\def\showappendix{true}\input main.tex"

poirot-jfp-sm-techreport.pdf: main.tex bibliography.bib sections/intro.tex sections/motivation.tex \
	sections/languages.tex sections/rules.tex sections/algorithm.tex sections/poly.tex \
	sections/monad.tex sections/evaluation.tex sections/related.tex commands.sty
	pdflatex -jobname="poirot-jfp-sm-techreport" -shell-escape "\def\techreportmode{true}\def\showappendix{true}\input main.tex"
	bibtex poirot-jfp-sm-techreport
	clear
	pdflatex -jobname="poirot-jfp-sm-techreport" -shell-escape "\def\techreportmode{true}\def\showappendix{true}\input main.tex"
	clear
	pdflatex -jobname="poirot-jfp-sm-techreport" -shell-escape "\def\techreportmode{true}\def\showappendix{true}\input main.tex"

# create pdf without bibs (fast)
haste:
	pdflatex -jobname="poirot-jfp" -shell-escape main

# remove tex objects
clean:
	rm -f *.log *.aux *.blg *.bbl *.out *~ *.cut *.aux *.cb *.cb2

# remove objects, including the pdf file
cleanall:
	 rm -f *.log *.aux *.blg *.bbl *.out *~ *.cut *.aux *.cb *.cb2 *.pdf

# check for things in the bib that aren't cited/used
# And checks for citations in the file that aren't in the bib
nocite:
	checkcites poirot-jfp


==> draft/details.tex <==
\subsection{Compositional Generator Programming}

With the coverage monad, people can verify their generators that build from primitive generators and combinators. We consider two style of data type generator programming:

\paragraph{Sized Combination} The test generator are parametric over the size of datatype, and people write a recursive function to build generator with larger size from smaller size via datatype constructors. \ZZ{How Qcheck recommend}

\begin{minted}[xleftmargin=5pt, numbersep=4pt, linenos = true, fontsize = \footnotesize, escapeinside=??]{OCaml}
let rec size_tree_gen (n: nat): unit -> int tree =
    match n with
    | 0 -> return Leaf
    | _ ->
        (return Leaf) ?$\oplus$?
        (fmap3 (fun r lt rt -> Node (r, lt, rt)) 
            int_gen (size_tree_gen (n-1)) (size_tree_gen (n-1)))

let tree_gen = bind nat_gen size_tree_gen 
\end{minted}

\ZZ{In Qcheck, the fix is also an combinator, maybe we should add it.}
\begin{minted}[xleftmargin=5pt, numbersep=4pt, linenos = true, fontsize = \footnotesize, escapeinside=??]{OCaml}    
    let fix f = 
        let rec f' n st = f f' n st in
        f'
    ?$\Code{fix}: \forall b\;\phi.(m{:}\nuot{nat}{\top}\sarr (n{:}\nuot{nat}{\vnu < m}\sarr\CM{b}{\phi(m)})) \sarr (n{:}\nuot{nat}{\top}\sarr\CM{b}{\phi(n)})$?
\end{minted}

\begin{minted}[xleftmargin=5pt, numbersep=4pt, linenos = true, fontsize = \footnotesize, escapeinside=??]{OCaml}
let tree_gen = bind nat_gen (fix 
    (fun (n: nat) self ->
        match n with
        | 0 -> return Leaf
        | _ ->
            (return Leaf) ?$\oplus$?
            (fmap3 (fun r lt rt -> Node (r, lt, rt)) 
                int_gen (self (n-1)) (self (n-1))))
)
\end{minted}


There is an interesting invariant that not use the datatype constructors but the API of an ADT.

\begin{minted}[xleftmargin=5pt, numbersep=4pt, linenos = true, fontsize = \footnotesize, escapeinside=??]{OCaml}
let set_gen = bind nat_gen (fix 
    (fun (n: nat) self ->
        match n with
        | 0 -> return Set.empty
        | _ ->
            (return Set.empty) ?$\oplus$?
            (fmap2 Set.insert int_gen (self (n - 1))))            
)
\end{minted}

\ZZ{I think these are not quite different from original Poirot.}

\paragraph{Generator Transformation}

A list generator can be defined from a tree generator:
\begin{minted}[xleftmargin=5pt, numbersep=4pt, linenos = true, fontsize = \footnotesize, escapeinside=??]{OCaml}
    let rec flatten (n : int) (tr : int tree) : int list =
        match tr with
        | Leaf -> []
        | Node (x, lt, rt) ->
            let (l1 : int list) = flatten (tree_num_node lt) lt in
            let (l2 : int list) = flatten (tree_num_node rt) rt in
            x :: list_concat l1 l2

    fmap (fun tr -> flatten (tree_num_node tr) tr) tree_gen 
\end{minted}

\ZZ{I have run this benchmark yesterday, there is an issue shown below.}

\subsection{Underapproximate parameter function types}

\paragraph{Intuition} Note that the bind and fmap function has a \emph{coverage combinator type} that has underapproximate parameter function types.
Technically, coverage combinator type is better than standard coverage function type when the implementation is deterministic (e.g., $\Code{flatten\_tree}$). The normal coverage function type of $\Code{flatten\_tree}$ would be of the form $x{:}\nuot{int\;tree}{\top}\sarr\rawnuut{int\;list}{\vnu = \I{flatten}(x)}$ where $\I{flatten}$ in qualifier logic needs to describe precisely how the implementation maps each tree into a list, which may extend the expressive power of qualifier logic and unnecessarily complicate matters. The coverage combinator type, on the other hand, can simply be $x{:}\nuut{int\;tree}{\top}\sarr\nuut{int\;list}{\top}$, which means ``if the input tree can cover all possible trees, the output list can also cover all possible lists''.

\paragraph{New typing rules}

We have new typing rules for monadic operators:

{\small
\mprooftr{43mm}
{$x$
}
{TReturn}
{$\Gamma \vdash \Code{return}\;v : \CM{b}{(\vnu = v)}$}
\quad
\mprooftr{53mm}
{
$\Gamma \vdash e : \CM{b_1}{\phi_1}$\quad
$\Gamma \vdash f : \rawnuut{b_1}{\phi_1}\sarr\CM{b_2}{\phi_2}$
}
{TBind}
% {$\Gamma \vdash \Code{return}\;v : \CM{b}{(\vnu = v)}$}
{$\Gamma \vdash \Code{bind}\;e\;f : \CM{b_2}{\phi_2}$}
}

We will have new typing rules for functions and applications containing coverage combinator types. The rule \textsc{TFunUnder} requires $x$ to be free in the type $\tau$. The rule \textsc{TAppUnder} introduces more constraints to deal with the application with underapproximate parameter types. Since the actual relation between each possible input value $a$ and coverage guarantee $\tau$ is hidden, we require the body of application $e$ to have type $\tau$ under all possible allowed assignments of $a$ (i.e., $a{:}\rawnuot{b}{\phi}$).

{\small
\mprooftr{38mm}
{
$\Gamma, x{:}\rawnuot{b}{\phi} \vdash e:\tau$
}
{TFunOver}
{$\Gamma \vdash \lambda x{:}b.e : x{:}\rawnuot{b}{\phi}\sarr\tau$}
\quad
\mprooftr{62mm}
{
$\Gamma, x{:}\rawnuut{b}{\phi} \vdash e : \tau \quad \Gamma \wellfoundedvdash \rawnuut{b}{\phi}\sarr\tau$
}
{\textcolor{red}{TFunUnder}}
{$\Gamma \vdash \lambda x{:}b.e : \rawnuut{b}{\phi}\sarr\tau$}
\\ \ \\ \ \\
\mprooftr{38mm}
{
$\Gamma \vdash v_1 : a{:}\rawnuot{b}{\phi}\sarr\tau_x$\quad
$\Gamma \vdash v_2 : \rawnuut{b}{\phi}$\quad
$\Gamma, x{:}\tau_x[a \mapsto v_2] \vdash e : \tau$
}
{TAppOver}
{$\Gamma \vdash \zlet{x}{v_1\ v_2}{e} : \tau$}
\quad
\mprooftr{58mm}
{
$\Gamma \vdash v_1 : a{:}\rawnuut{b}{\phi}\sarr\tau_x$\\
$\Gamma \vdash v_2 : \rawnuut{b}{\phi}$\\
$\Gamma, a{:}\rawnuot{b}{\phi}, \I{tmp}{:}\nuut{unit}{a = v_2}, x{:}\tau_x \vdash e : \tau$
}
{\textcolor{red}{TAppUnder}}
{$\Gamma \vdash \zlet{x}{v_1\ v_2}{e} : \tau$}
}

\paragraph{Explanation} Following the intuition provided in the beginning of the section, we should allowing the under-parameter function type to \emph{hidden} precise reachability mapping relation, which means we requires the binding variables $x$ is not free variable in the return type of $x{:}\rawnuut{b}{\phi}\sarr\tau$. This precision lose can lead a potential soundness problem as discussed in incorrectness workshop.

 As an example, consider the
function type
$\tau \equiv \nuut{int}{\top}\sarr\nuut{int}{1 \leq \vnu \leq 2}$ with
underapproximate parameter types, and the following two valid
implementations of this type which are the same:
\begin{minted}[xleftmargin=10pt, numbersep=4pt, linenos = true, fontsize = \small, escapeinside=!!]{ocaml}
let f (x: int) = if x > 0 then 1 else 2
let g (x: int) = if x > 0 then 1 else 2
\end{minted}
%
\noindent The following program that uses two functions
$\Code{f}$ and $\Code{g}$ of type $\tau$:
\begin{minted}[xleftmargin=10pt, numbersep=4pt, linenos = true, fontsize = \small, escapeinside=!!]{ocaml}
  let client =
  let (x: int) = int_gen () in (f x) - (g x) in x
\end{minted}
Notice that, the client cannot return any value other than $0$, although from types we may believe it can be $-1$, $0$, or $1$, that are all combination of difference of values in the range $[1,2]$. Actually, the return value of the function decide the sign of the $x$. For example, when $f\;x$ returns $2$, $x$ is will lose the coverage of all positive integers.

In general, as a treat-off that we lose the precision, we cannot figure out the actually relation of inputs and outputs, thus we cannot precisely analysis this coverage change. Alternatively, we should guarantee the value used linearly during under-parameter function application.

\ZZ{Concern:} I find that it is kind of annoying to add these constraints into type context, also, it may break the EPR constraints, where $a$ is overapproximated, which leads more quantifier alternation. For example

\begin{minted}[xleftmargin=5pt, numbersep=4pt, linenos = true, fontsize = \footnotesize, escapeinside=??]{OCaml}
fun (tr: int tree) ->
    let (n: int) = tree_num_node tr in
    let (tmpf: int tree -> int list) = flatten n in
    (* Typing here:*)
    ?$\Code{tr}{:}\nuut{tree}{\top}, \Code{n}{:}\nuut{int}{\I{numNode}(\Code{tr}) = \vnu}, \Code{tmpf}{:}(\nuut{tree}{\I{numNode}(v) = \Code{n}}\sarr\nuut{list}{\I{len}(v) = \Code{n}})$?
    ?$\Code{tr'}{:}\nuot{tree}{\I{numNode}(v) = \Code{n}}, \Code{tmp}{:}\nuut{unit}{\Code{tr = tr'}},$?
    let (l: int list) = tmpf tr in
    ...
\end{minted}

The qualifier of $\Code{tr'}$ contains $\Code{n}$, which is a $\exists\forall$ pattern. Original coverage type already allowing $\forall\exists$, then this may cause arbitrary quantifier alternation.

\ZZ{Syntactic Linear check doesn't work:} The naive linear check doesn't work:
{\small\begin{align}
    x{:}\nuut{int}{\vnu > 0}, y{:}\nuut{int}{y = x + 1}, 
\end{align}}\noindent
when $y$ is used, the value of $x$ is also fixed. The $y$ and $x$ is semantically related.

\ZZ{Data-flow context} Consider to introduce a data-flow context $\Psi \doteq \mathcal{P}(x\times x)$ contains all used variables and all dependencies variables with underapproximate type. At each function application and pattern match, it add new dependency into the context. A used variable context $\Pi$ contains all used variables. $\Psi(V)$ will calculate the closure of all dependent variables of variable set $V$.

{\small
\mprooftr{48mm}
{
$\Psi ~|~ \Pi ~|~ \Gamma \vdash v_1 : \rawnuut{b}{\phi}\sarr\tau_x$\\
$\Psi ~|~ \Pi ~|~ \Gamma \vdash v_2 : \rawnuut{b}{\phi}$\\
$\Psi(\Pi) \cap \Psi(\Code{FV}(v_2)) =\emptyset$\\
$\Psi ~|~ \Pi\cup\Code{FV}(v_2) ~|~ \Gamma, x{:}\tau_x \vdash e : \tau$
}
{\textcolor{red}{TAppUnder}}
{$\Psi ~|~ \Pi ~|~ \Gamma \vdash \zlet{x}{v_1\ v_2}{e} : \tau$}
\quad
\mprooftr{66mm}
{
$\Psi ~|~ \Pi ~|~ \Gamma \vdash v_1 : a{:}\rawnuot{b}{\phi}\sarr\tau_x$\quad
$\Psi ~|~ \Pi ~|~ \Gamma \vdash v_2 : \rawnuut{b}{\phi}$\\
$\Psi \cup \{(y, x) ~|~ y \in \Code{FV}(v_2) \} ~|~ \Pi ~|~ \Gamma, x{:}\tau_x[a \mapsto v_2] \vdash e : \tau$
}
{TAppOver}
{$\Psi ~|~ \Pi ~|~ \Gamma \vdash \zlet{x}{v_1\ v_2}{e} : \tau$}
}

Note that, the under-application won't create dependency relation, the precision lose means the they are not data-flow dependent.

% The date-dependent relation $\Gamma \vdash x \rightharpoonup x$ is defined as the following:

% {\small
% \mprooftr{28mm}
% {
% $(x, \rawnuut{b}{\phi}) \in \Gamma$
% }
% {DepSelf}
% {$\Gamma ~|~ x \rightharpoonup x$}
% \mprooftr{58mm}
% {
% $(z, \rawnuut{b}{\phi}) \in \Gamma$\quad
% $y \in \Code{FV}(\phi)$\quad
% $\Gamma ~|~ x \rightharpoonup y$
% }
% {DepSelf}
% {$\Gamma ~|~ x \rightharpoonup z$}
% }




\subsection{Meta theorem}

\paragraph{New typing denotations}

\begin{align*}
    &\denot{\rawnuot{b}{\phi}}  &&\doteq \{ v ~|~ \emptyset \basicvdash v : b \land \phi[\vnu\mapsto v] \}\\
    &\denot{\rawnuut{b}{\phi}}  &&\doteq \{ e ~|~ \emptyset \basicvdash e : b \land \forall v{:}b. \phi[\vnu\mapsto v] \impl \mstep{e}{v} \}\\
    &\denot{x{:}\tau_x\sarr\tau}  &&\doteq \{ e ~|~\emptyset \basicvdash e : \eraserf{x{:}\tau_x\sarr\tau} \land \exists v{:}\eraserf{x{:}\tau_x\sarr\tau}. \mstep{e}{v} \land \forall v_x\in\denot{\tau_x}. v\; v_x \in \denot{\tau[x\mapsto v_x]} \}\\
    & &&\text{new type denotation: } \\
    &\denot{\rawnuut{b}{\phi}\sarr\tau}  &&\doteq \{ e ~|~\emptyset \basicvdash e : b\sarr\eraserf{\tau} \land \exists v{:}\eraserf{x{:}\tau_x\sarr\tau}. \mstep{e}{v} \land \forall e_x\in\denot{\rawnuut{b}{\phi}}. v\; e_x \in \denot{\tau} \}\\
    & && \textcolor{DeepGreen}{\text{the assignment of $x$ cannot be a value which needs to have a coverage type;}} \\
    & && \textcolor{DeepGreen}{\text{thus we cannot replace a term directly into the qualifier of types.}}
\end{align*}

\ZZ{Some technical details, may not shown in the main paper. I am not satisfying about the old type context denotation, although it is correct, but I believe there should be a better way. Here is the old one, where we don't have a standalone definition of denotation of type context}

{\small
\begin{alignat*}{2}
    \denot{\tau}_{\emptyset} &\doteq \denot{\tau}
    \\ \denot{\tau}_{x{:}\tau_x, \Gamma} &\doteq \{ e ~|~
    \forall v_x \in \denot{\tau_x}, \zlet{x}{v_x}{e} \in
    \denot{\tau [x\mapsto v_x]}_{\Gamma [x\mapsto v_x]} \} \qquad\qquad\qquad\ \ \text{ if $\tau
      \equiv \rawnuot{b}{\phi}$} \\
      \denot{\tau}_{x{:}\tau_x,
      \Gamma} &\doteq \{ e ~|~ \exists \hat{e}_x \in
    \denot{\tau_x}, \forall e_x \in \denot{\tau_x},
    \zlet{x}{e_x}{e} \in \bigcap_{\hat{e}_x \hookrightarrow^*
      v_x} \denot{\tau
    [x\mapsto v_x]}_{\Gamma [x\mapsto v_x]} \}
    \quad \text{ otherwise}
\end{alignat*}}\noindent

\ZZ{Here is my proposal}

{\small\begin{alignat*}{2}
    \denot{\Gamma} &\in \mathcal{P}(\sigma \times \mathcal{P}(\sigma))
\end{alignat*}}\noindent
which indicates a $\forall\exists$ prefix. A property $\phi$ is correct under type context $\Gamma$ iff
{\small
\begin{alignat*}{2}
    \forall (\sigma, \Sigma) \in \denot{\Gamma}. \exists \sigma' \in \Sigma. \sigma(\sigma'(\phi))
\end{alignat*}}\noindent
The the $\hat{e}$ can be split from the denotation of type context, where we say $e \in \denot{\tau}$ under type context iff
{\small\begin{alignat*}{2}
    % \forall (\sigma, \Sigma) \in \denot{\Gamma}. \exists \hat{\Sigma}. \hat{\Sigma} \subseteq \Sigma \land (\forall \hat{\sigma} \in \hat{\Sigma}. \exists \sigma' \in \Sigma'. \sigma(\sigma'(e)) \in \denot{\sigma(\hat{\sigma}(\tau))})
    \forall (\sigma, \Sigma) \in \denot{\Gamma}. \exists \hat{\Sigma}. \hat{\Sigma} \subseteq \Sigma \land \bigoplus_{\sigma' \in \Sigma'} \sigma(\sigma'(e)) \in \bigcap_{\hat{\sigma} \in \hat{\Sigma}}  \denot{\sigma(\hat{\sigma}(\tau))}
\end{alignat*}}\noindent
The $\hat{\Sigma}$ works the same as $\hat{e}$.

\ZZ{I have tried to prove it this weekend, I believe it can make the Coq proof be clearer.}

\subsection{Typing algorithm}

{\small
\begin{prooftree}
\hypo{
\parbox{72mm}{\center
  $\Gamma \vdash v_1 \typeinfer \rawnuut{b}{\phi}\sarr\tau_x$\quad
  $\Gamma \vdash v_2 \typecheck \rawnuut{b}{\phi}$\quad
  $\Gamma, \text{linear check}, x{:}\tau_x \vdash e \typeinfer \tau$ \quad
$\tau' = \existsop(x{:}\tau_x, \tau)$ \quad $\Gamma \vdash \tau'$
}
}
\infer1[\textsc{SynAppBase}]{
\Gamma \vdash \zlet{x}{v_1\ v_2}{e} \typeinfer \tau'
}
\end{prooftree}
}

\subsection{Evaluation}

\begin{enumerate}
    \item Re-implement some of old PLDI benchmarks using combinators.
    \item Generator transformation over different datatypes.
    \item ADT APIs combination, verify coverage of subset of APIs.
\end{enumerate}

I don't want to add ``combinator implementation'' into benchmarks, which involve a qualifier polymorphism ($\forall \phi$) in many monadic combinators in QCheck library (e.g., $\Code{union}$):
\begin{align*}
    \Code{union} : \forall \phi_1\;\phi_2.\CM{b}{\phi_1} \sarr \CM{b}{\phi_2} \sarr \CM{b}{(\phi_1 \lor \phi_2)}
\end{align*}\noindent
Verifying the implementation of these combinators need to derive verification condition in higher-order logic, which seems out of the expressive power of SMT solver. Also, the actual implementation of these combinators are typically stateful.
Maybe we can only make them as builtin combinators, and verify the generators (e.g., list gen) that written using these combinators. We don't need to modify the types, but can hard code the builtin combinators into type system.

==> draft/proposal.tex <==
\section{Introduction}

We further extend our coverage type checker to support more scalable property-based testing, including both monadic PBT libraries (e.g., QCheck) and real-world applications built upon them. To support this, we enhance our type system with polymorphism over both types and qualifiers.

\section{Polymorphic Coverage Type}

\paragraph{Type polymorphism} Standard.
\paragraph{Qualifier polymorphism} For bind function, the output coverage is depends on input coverage. We need to express ``for all possible coverage'', it cannot be $\top$ qualified coverage which is a super type instead of standard refinement type qualifier. 
\paragraph{Typing algorithm for qualifier polymorphism} 


\section{Monadic Coverage Type}

\paragraph{Definition of Coverage Monads} 

\paragraph{Interesting examples} 

\section{New Evaluations}

\section{Extension Proposal}

People typically use a monadic style to write test generators, where complicated test generators are constructed from simpler test generators and generator combinators. We extend coverage types with \emph{coverage monads} and \emph{coverage combinator types} to support this monadic programming style. The following subsection introduces the proposed extension with examples.

\subsection{Coverage Monad}

We introduce the \emph{coverage monad} $\Murt{b}{\phi}$, which indicates the coverage guarantee $\phi$ of a test generator over datatype $b$. This monad is a shortcut for the a coverage refinement type:
\begin{align*}
    \Murt{b}{\phi} &\doteq  x{:}\urt{\Unit}{\top}\sarr\urt{b}{\phi}
    \\\M{\tau} &\doteq x{:}\urt{\Unit}{\top}\sarr\tau
    \\\M{t} &\doteq \Code{unit}\sarr t
\end{align*}\noindent

We add polymorphic basic type $\forall t.\tau$ and polymorphic method predicate $\forall (p{:}t).\tau$.

{\small
    \begin{alignat*}{2}
    \text{\textbf{Type Variable}}& \quad &  \quad &  \textcolor{red}{X, Y, Z, ...} \\
    \text{\textbf{Base Type Variable}}& \quad &\quad &  \textcolor{red}{X_b, Y_b, Z_b, ...} \\
    \text{\textbf{Type Constructor}}& \quad & C ::= \quad &    \Code{list} ~|~ \Code{tree} ~|~ \ldots \\
    \text{\textbf{Basic Types}}& \quad & b,t ::= \quad & \Code{unit} ~|~ \Code{bool} ~|~ \Code{nat} ~|~ \Code{int} ~|~ C \;\overline{t} ~|~ t\sarr t ~|~ X ~|~ \forall X.t ~|~ \forall X_b.t \\
    \text{\textbf{Refinement Types}}& \quad &\tau  ::= \quad & \urt{b}{\phi} ~|~ \ort{b}{\phi} ~|~ x{:}\tau\sarr\tau ~|~  \\
    & \quad & \quad & \textcolor{red}{\forall X.\tau ~|~ \forall X_b.\tau ~|~ \forall p{:}(\overline{b_i}\sarr \Bool).\tau} \\
    \text{\textbf{Type context}}& \quad &\Gamma  ::= \quad & \emptyset ~|~ \Gamma, x{:}\tau ~|~ \Gamma, p{:}t ~|~ \Gamma, X ~|~ \Gamma, X_b
  \end{alignat*}
}

\paragraph{Kinds} Different from the standard kind that just distinguish the kind of proper types and type constructors (e.g., $\Code{list}: \star \sarr \star_b$), we additional distinguish ``proper base types'' ($\star_b$) and ``arbitrary proper types'' ($\star$), where the later one can include function types. We always use $b$ to refer proper base types and $t$ to refer all possible base types. Thus, the base refinement type $\urt{b}{\phi}$ and $\ort{b}{\phi}$ can only qualify over base proper types. The polymorphic type variable must be instantiated into a concrete type with the same kind.

\newcommand{\gen}[1]{{#1}\;\Code{gen}}

\begin{minted}[xleftmargin=5pt, numbersep=4pt, linenos = true, fontsize = \footnotesize, escapeinside=??]{OCaml}
    let oneof f = fun () -> f (nat_gen ()) ()
    val oneof: ?$\forall X{:}\kb.(\Nat\sarr\M{X}) \sarr \M{X}$?
    ?$\vdash \Code{oneof} : \forall X{:}\kb. \forall p{:}(\Nat\sarr X \sarr \Bool).$?
        ?$(i{:}\Nat\sarr\Murt{X}{p(i,\vnu)})\sarr \Murt{X}{\exists i{:}\Nat. p(i,\vnu)}$?

    let nil_gen = fun _ -> fun () -> err
    val nil_gen: ?$\forall X{:}\kb.\Nat\sarr\M{X}$?
    ?$\vdash \Code{nil\_gen} : \forall X{:}\kb.i{:}\Nat\sarr\Murt{X}{\bot})$?
    
    let cons_gen (g: 'a gen) (l: nat -> 'a gen) = 
        fun i -> if i == 0 then g else l (i - 1)
    val cons_gen: ?$\forall X{:}\kb.\M{X}\sarr(\Nat\sarr\M{X})\sarr(\Nat\sarr\M{X})$?
    ?$\vdash \Code{cons\_gen} : \forall X{:}\kb. \forall p_0{:}(X \sarr \Bool).\forall p{:}(\Nat\sarr X \sarr \Bool).$?
        ?$\Murt{X}{p_0(\vnu)} \sarr (i{:}\Nat\sarr\Murt{X}{p(i,\vnu)})\sarr (i{:}\Nat\sarr\Murt{X}{(i = 0 \land p_0(\vnu) \lor i > 0 \land p(i-1,\vnu)})$?
\end{minted}

\paragraph{Benchmarks 1: Tezos} Block chain generator.

\begin{minted}[xleftmargin=5pt, numbersep=4pt, linenos = true, fontsize = \footnotesize, escapeinside=!!]{OCaml}
    type shell_header = {branch : Hash.t}
    type operation = {shell : shell_header; proto : Bytes.t}

    let operation_proto_gen = small_string ?gen:None
    !$\vdash \M{\urt{\String}{\len(\vnu) < 100}}$!
    
    let operation_mock_proto_gen =
        let len_gen = frequency (fun i -> if i == 0 then (9, return 0)
                                          else if i == 1 then (1, int_range 0 31)
                                          else return err) in
        string_size ?None len_gen
    !$\vdash \M{\urt{\String}{\len(\vnu) < 31}}$!

    let operation_gen block_hash_gen =
        prod_block_hash_gen >>= (fun branch ->
            operation_proto_gen >|= (fun proto ->
                {shell = {branch}; proto = Bytes.of_string proto}))
    !$\vdash \forall p{:}\Code{\Byte}\sarr\Bool.\M{\urt{\Byte}{p(\vnu)}}\sarr \M{\urt{\Code{operation}}{\len(\Code{\vnu.shell.branch}) < 100 \land p(\Code{\vnu.proto})}}$!
\end{minted}

\begin{minted}[xleftmargin=5pt, numbersep=4pt, linenos = true, fontsize = \footnotesize, escapeinside=!!]{OCaml}
    (* Rational number between 0 to 1*)
    let q_in_0_1 =
        let q = int_range 1 max_int in
        let p = int_range 0 q in
        Q.make p q
    !$\vdash \M{\urt{\Int\times\Int}{0 \leq_Q \vnu \leq_Q 1}}$!

    type priority = High | Medium | Low of (int * int) list
    
    let priority_gen () =
        (oneofl [High; Medium; Low []]) >>= (fun top_prio_value ->
          match top_prio_value with
          | High -> return High
          | Medium -> return Medium
          | Low _ -> small_list (q_in_0_1 ()) >|= (fun weights -> Low weights))
    !$\vdash \M{\urt{\Code{priority}}{\I{qlen}(\vnu) < 100}}$!
\end{minted}

\begin{minted}[xleftmargin=5pt, numbersep=4pt, linenos = true, fontsize = \footnotesize, escapeinside=!!]{OCaml}
    (** Trees representing the shape of the chain. The root is the common
      ancestor of all blocks, like this:

                      head3
                        /
         head1  head2  .
            \       \ /
             .       .
              \     /
              ancestor
    *)
    (* all elements in a tree should be different*)
    type 'a tree =
    | Leaf of 'a
    | Node1 of ('a * 'a tree)
    | Node2 of ('a * 'a tree * 'a tree)

    (** A tree generator. Written in a slightly unusual style because it
      generates all values beforehand, to make sure they are all different.
      This is a property we want for trees of blocks. To do so,
      this generator first generates a list of elements [e1; e2; e3; e4; e5; e6]
      and then progressively splits this list to build the subtrees.

      For example it takes [e1] for the root value and then splits
      the rest into [e2; e3] and [e4; e5; e6]. Then it recurses, sending
      [e2; e3] as values to create the left subtree and [e4; e5; e6] to
      create the right subtree.

      This generator takes as parameter an optional list of blocks. If
      they are given, they are used to build the tree; otherwise fresh
      ones are generated. *)
let rec tree_gen ?(blocks: !$\ort{\List{\Code{block}}}{\len(\vnu) > 0 \land \uniq(\vnu)}$!) () =
    match blocks with
    | [] -> return None
    | [x] -> return (Some (Tree.Leaf x))
    | x :: xs -> 
        let g1 =
            let* sub = tree_gen xs in
            match sub with    
            | None -> return (Some (Tree.Leaf x))
            | Some sub -> return (Some (Tree.Node1 (x, sub))) in
        let g2 =
            let* n = int_bound (List.length xs - 1) in
            let left, right = List.split_n n xs in
            let* left = tree_gen left and* right = tree_gen right in
              match (left, right) with
              | None, None -> return (Some (Tree.Leaf x))
              | None, Some sub | Some sub, None -> return (Some (Tree.Node1 (x, sub)))
              | Some left, Some right -> return (Some (Tree.Node2 (x, left, right))) in
        union g1 g2
!$\vdash \Code{blocks}{:}\ort{\List{\Code{block}}}{\len(\vnu) > 0 \land \uniq(\vnu)} \sarr \M{\urt{\Tree[\Code{block}]}{\I{numElem}(\vnu) = \len(\Code{blocks})}}$!
\end{minted}

\paragraph{Benchmarks 2: Xen API} File descriptor generator.

\begin{minted}[xleftmargin=5pt, numbersep=4pt, linenos = true, fontsize = \footnotesize, escapeinside=!!]{OCaml}
type file_kind = S_BLK | S_CHR | S_DIR | S_FIFO | S_LNK | S_REG | S_SOCK
type fd = { size: int; 
           delay_read: Delay.t option; 
           delay_write: Delay.t option; 
           kind: file_kind }
let all_file_kind = [S_BLK; S_CHR; S_DIR; S_FIFO; S_LNK; S_REG; S_SOCK]
let file_kind_gen = oneofl all_file_kind
!$\vdash \M{\urt{\Code{file\_kind}}{\top}}$!
let testable_file_kind_gen = onefl (List.filter testable all_file_kind)
!$\vdash \M{\urt{\Code{file\_kind}}{\I{testable}(\vnu)}}$!

(** [select_fd_spec] defines a behaviour for a select input: a file descriptor kind and how long before any event happens on it *)
type select_fd_spec = {kind: file_kind; wait: float}

let timeouts = oneofl [0.0; 0.001; 0.1; 0.3]
!$\vdash \M{\urt{\Code{float}}{\I{timeout}(\vnu)}}$!

let select_fd_spec =
  let+ kind = fst testable_file_kind and+ wait = timeouts in
  {kind; wait= (if has_immediate_timeout kind then 0. else wait)}
!$\vdash \M{\urt{\Code{select\_fd\_spec}}{\I{wf\_fd\_spec}(\vnu)}}$!

let file_list =
  let* size_bound = frequencya [|(4, 0); (4, 2); (2, 10); (1, 100)|] in
  let size_gen = int_bound size_bound in
  let repeated_list =
    let* size = size_gen in
    list_repeat size select_fd_spec
  in
  (* generates 2 kinds of lists:
     - lists that contain only a single file kind
     - lists that contain multiple file kinds

     This is important for testing [select], because a single
       [Unix.S_REG] would cause it to return immediately,
       making it unlikely that we're actually testing the behaviour for other file descriptors.
  *)
  oneof [repeated_list; list_size size_gen select_fd_spec]
!$\vdash \M{\urt{\List[\Code{select\_fd\_spec}]}{\I{wf\_fd\_spec\_list}(\vnu) \land \len(\vnu) < 100}}$!

let total_delays = oneofl [0.001; 0.01; 0.1; 0.4]
!$\vdash \M{\urt{\Code{float}}{\I{total\_delays}(\vnu)}}$!

let ocaml_unix_buffer_size = 65536

let sizes =
  Gen.oneofa
    [|
       0
     ; 1
     ; 100
     ; 4096
     ; ocaml_unix_buffer_size - 1
     ; ocaml_unix_buffer_size
     ; ocaml_unix_buffer_size + 1
     ; 2 * ocaml_unix_buffer_size
     ; (10 * ocaml_unix_buffer_size) + 3
    |]
!$\vdash \M{\urt{\Int}{\I{wf\_size}(\vnu)}}$!

let fd_gen =
  (* order matters here for shrinking: shrink timeout first so that shrinking completes sooner! *)
  let* total_delay = total_delays
  and* size = sizes
  and* kind = testable_file_kind in
  let size = if kind = Unix.S_BLK then 512 else size in
  let* delay = delay_of_size total_delay size in
  (* see observations.ml, we can't easily change size afterwards *)
  return { size; delay_read = delay; delay_write = Some delay; kind }
!$\vdash \M{\urt{\Code{fd}}{\I{wf\_fd}(\vnu)}}$!
\end{minted}

\paragraph{Benchmarks 3: Vellvm} Undefined symbolic values generators.

\begin{minted}[xleftmargin=5pt, numbersep=4pt, linenos = true, fontsize = \footnotesize, escapeinside=!!]{OCaml}
(* LLVM types *)
type typ =
    | TYPE_I of int
    | TYPE_Void
    | TYPE_Vector of int * typ 
    | TYPE_Array of int * typ
    | TYPE_Others

(* LLVM dynamic values *)
type dvalue =
    | DVALUE_I of int * int
    | DVALUE_None
    | DVALUE_Vector of typ * list dvalue
    | DVALUE_Array of typ * list dvalue
    | DVALUE_Others

let small_gen = int_range 0 10000
!$\vdash \M{\urt{\Int}{0 \leq \vnu \leq 10000}}$!
    
let g_i1 = bool_gen >|= (fun v ->
               DV.UVALUE_I (P.of_int 1, (if v then Z.one else Z.zero))) G.bool
!$\vdash \M{\urt{\Int}{0 \leq \vnu \leq 10000}}$!

(* undefined symbolic values (uvalue) which is a subset of dvalue, see paper and note: https://github.com/vellvm/vellvm/blob/38b549eae8bbf1a66c32b99104a845690a40cf69/doc/intern/notes.org#L155 *)
let rec gen_uvalue (t: typ): dvalue M.t = 
  match t with
  | TYPE_I i ->
     (match i with
        | 1 -> g_i1 | ...
        | _ -> err)
  | TYPE_Void -> return UVALUE_None
  | TYPE_Vector (sz, ty) ->
     let list_ts = G.list_size (return sz) (gen_uvalue ty) in
     list_ts >|= (fun l -> DV.UVALUE_Vector (t, l))
  | TYPE_Array (sz, ty) ->  
     let list_ts = G.list_size (return sz) (gen_uvalue ty) in
     list_ts >|= (fun l -> DV.UVALUE_Array (t, l))
  | TYPE_Others -> err
!$\vdash \M{\urt{\Code{dvalue}}{\I{uvalue}(\vnu) \land 0 \leq \I{maxInt}(\vnu) \leq 1000}}$!
\end{minted}

\paragraph{Benchmarks 4: Herdtools7} Type and expression generator. 

\begin{minted}[xleftmargin=5pt, numbersep=4pt, linenos = true, fontsize = \footnotesize, escapeinside=!!]{OCaml}

type config = { e_literal: bool; e_var: bool; e_unop: bool; 
                e_binop: bool; e_tuple: bool; e_cond: bool; e_slice: bool}

let e_literal = ...
let e_var = ...

let expr (config: config): expr M.t =
    fix @@ fun expr n ->
        let n = if n <= 0 then 0 else n - 1 in
        oneof (filter [
              (if config.e_literal then e_literal else None);
              (if config.e_var then Some e_var else None);
              (if config.e_unop && n >= 0 then e_unop expr n else None);
              (if config.e_binop && n >= 2 then e_binop expr n else None);
              (if config.e_tuple && n >= 2 then Some (e_tuple expr n) else None);
              (if config.e_cond && n >= 3 then Some (e_cond expr n) else None);
              (if config.e_slice && n >= 1 then Some (e_slice expr n) else None);
            ])
!$\vdash \Code{c{:}config}\sarr\M{\urt{\Code{expr}}{\Code{c.e\_literal}\iff\I{hasLiteral}(\vnu) \land ...}}$!
// type is similar
\end{minted}

\paragraph{Benchmarks 5: Zipperposition} three kinds of typed term generator: HigherOrder, LambdaFreeHigherOrder and FirstOrder. I have to say, there is no meaningful coverage for these functions, because it is very incomplete.

\begin{minted}[xleftmargin=5pt, numbersep=4pt, linenos = true, fontsize = \footnotesize, escapeinside=!!]{OCaml}
type id = string
type builtin_ty = TType | Prop | Term | Rat | Int | Real

type ty = private
  | TBuiltin of builtin_ty
  | TVar of ty * string
  | TDB of int
  | TApp of id * ty list (** parametrized type *)
  | TFun of ty list * ty (** Function type (left to right, no left-nesting) *)
  | TForall of ty (** explicit quantification using De Bruijn index *)

type term = private
  | AppBuiltin of op * term list
  | DB of int (** Bound variable (De Bruijn index) *)
  | Var of ty * string (** Term variable *)
  | Const of id (** Typed constant *)
  | App of term * term list (** Application to a list of terms (cannot be left-nested) *)
  | Fun of ty * term (** Lambda abstraction *)

let tterm = TBuiltin Term
let tint = TBuiltin Int
let ttype = TBuiltin TType
let tvar x = TVar (ttype, "a")

let ty_gen =
  let g = fix
      (fun self n ->
         let sub = self (n-1) in
         if n<=0 then base
         else frequency
             [ 1, (list_repeat 1 sub) >|= (fun args -> TApp ("list", args))
             ; 1, (list_repeat 2 sub) >|= (fun args -> TApp ("prod", args))
             ; 1, (list_size (1--2) sub) >|= (fun param ->
                sub >|= (fun ret -> TFun (param, ret)))
             ; 3, (oneofl [tterm; tint; tvar "a"; tvar "b";])
             ])
  in
  1 -- 4 >>= g

let fo_gen n =
    let base = oneofl [a;b;c;d;e;x;y;z] in
    let gen =
      fix
        (fun self n ->
           let self = self (n-1) in
           if n<=0 then base
           else (
             let fo_list = [
               3, base;
               1, map2 f self self;
               1, map2 sum self self;
               1, map g self;
               1, map h self;
               1, map3 ite self self self;
             ] in
             frequency fo_list
           ))
    in
    (1 -- n) >>= gen
\end{minted}

\paragraph{Well-formedness} In order to instantiate the quantified method predicates, we need to guarantee these predicates are exactly qualifier of some parameter type.

\newcommand{\baset}[1][]{\mathbf{base}({#1})}
\begin{align*}
    \baset[\Code{unit} ~|~ \Code{bool} ~|~ \Code{nat} ~|~ \Code{int} ~|~ \overline{t}\;C ] = \true
\end{align*}

\begin{prooftree}
\hypo{\Gamma, p{:}t, x{:}\ort{b}{p(\vnu)} \wfvdash \tau}
\infer1[\textsc{WFPolyOverArr}]{ 
\Gamma \wfvdash \forall p{:}t.x{:}\ort{b}{p(\vnu)}\sarr\tau
}
\end{prooftree}
\quad
\begin{prooftree}
\hypo{\Gamma, x{:}\ort{b}{p(\vnu)} \wfvdash \tau}
\infer1[\textsc{WFOverArr}]{ 
\Gamma \wfvdash x{:}\ort{b}{p(\vnu)}\sarr\tau
}
\end{prooftree}
\quad
\begin{prooftree}
\hypo{\Gamma, (y{:}\tau_1\sarr\tau_2) \wfvdash \tau}
\infer1[\textsc{WFArrArr}]{ 
\Gamma \wfvdash x{:}(y{:}\tau_1\sarr\tau_2)\sarr\tau
}
\end{prooftree}

\begin{minted}[xleftmargin=5pt, numbersep=4pt, linenos = true, fontsize = \footnotesize, escapeinside=??]{OCaml}
    (* Builtin generators *)

    ?$\vdash \Code{bool\_gen}: \Murt{\Int}{\top}$?
    ?$\vdash \Code{int\_gen}: \Murt{\Bool}{\top}$?
\end{minted}

We consider to add the following Qcheck $18$ APIs into our benchmarks:
\begin{minted}[xleftmargin=5pt, numbersep=4pt, linenos = true, fontsize = \footnotesize, escapeinside=??]{OCaml}
    (* Monadic conbinators *)
    
    let return x = fun () -> x
    ?$\vdash \Code{return}: \forall X{:}\kb.x{:}X \sarr \Murt{b}{\vnu = x}$?
    
    let bind gen f = fun () -> f (gen ()) ()
    ?$\vdash \Code{bind}: \forall X_1\;X_2{:}\kb.\forall p_1{:}(X_1\sarr\Bool).\forall p_2{:}(X_1\sarr X_2\sarr\Bool).$?
        ?$\Murt{X_1}{p_1(\vnu)} \sarr (x{:}\ort{X_1}{p_1(\vnu)}\sarr\Murt{X_2}{p_2(x, \vnu)}) \sarr \Murt{X_2}{\exists x. p_1(x)\land p_2(x, \vnu)}$?
    
    let fmap f gen = fun () -> f (gen ())
    ?$\vdash \Code{fmap}: \forall X_1\;X_2{:}\kb.\forall p_1{:}(X_1\sarr\Bool).\forall p_2{:}(X_1\sarr X_2\sarr\Bool).$?
        ?$(x{:}\ort{X_1}{p_1(\vnu)}\sarr\urt{X_2}{p_2(x, \vnu)}) \sarr \Murt{X_1}{p_1(\vnu)} \sarr \Murt{X_2}{\exists x. p_1(x)\land p_2(x, \vnu)}$?

    let fmap2 f gen1 gen2 = fun () -> f (gen1 ()) (gen2 ())
     ?$\vdash \Code{fmap}: \forall X_1\;X_2\;X_3{:}\kb.\forall p_1{:}(X_1\sarr\Bool).\forall p_2{:}(X_2\sarr\Bool).\forall p_3{:}(X_1\sarr X_2\sarr X_3\sarr\Bool).$?
        ?$(x{:}\ort{X_1}{p_1(\vnu)}\sarr y{:}\ort{X_2}{p_2(\vnu)}\sarr\urt{X_3}{p_3(x, y, \vnu)}) \sarr$?
        ?$\Murt{X_1}{p_1(\vnu)} \sarr \Murt{X_2}{p_2(\vnu)} \sarr \Murt{X_3}{\exists x\;y. p_1(x)\land p_2(y) \land p_3(x,y,\vnu)}$?

    let union gen1 gen2 = 
        bool_gen (function true -> gen1 | false -> gen2)
    ?$\vdash \Code{union}: \forall X{:}\kb.\forall p_1\;p_2{:}(b\sarr\Bool).\Murt{b}{p_1(\vnu)} \sarr \Murt{b}{p_2(\vnu)} \sarr \Murt{b}{p_1(\vnu)\lor p_2(\vnu)}$?

    let fix f = 
        let rec f' n st = f f' n st in f'
    ?$\Code{fix}: \forall X{:}\kb\forall (p{:}\Nat\sarr b\sarr\Bool).$?
        ?$(m{:}\Nat\sarr (n{:}\ort{\Nat}{\vnu < m}\sarr\Murt{b}{p(n, \vnu)}) \sarr \Murt{b}{p(m, \vnu)}) \sarr (m{:}\Nat\sarr\Murt{b}{p(m, \vnu)})$?
\end{minted}

\begin{minted}[xleftmargin=5pt, numbersep=4pt, linenos = true, fontsize = \footnotesize, escapeinside=??]{OCaml}
    (*inonline lin *)

    let int_bound (n: int): unit -> int =
        if n < 0 then err
        else fmap (fun r -> r mod (n+1)) int_gen
    ?$\vdash \Code{int\_bound}: n{:}\ort{\Int}{\vnu \geq 0}\sarr\Murt{\Int}{0 \leq \vnu \leq n}$?
    
    let int_range (a: int) (b: int) =
        if b < a then err
        else fmap (fun x -> a + x)  (int_bound (b-a))
    ?$\vdash \Code{int\_range}: a{:}\Int\sarr b{:}\ort{\Int}{a \leq \vnu}\sarr\Murt{\Int}{a \leq \vnu \leq b}$?

    let nat =
        bind (int_bound 10) (fun p ->
            if p < 5 then int_bound 10
            else if p < 8 then int_bound 100
            else if p < 9 then int_bound 1000
            else int_bound 10000)
    ?$\vdash \Code{nat}: \Murt{\Int}{0 \leq \vnu \leq 10000}$?
    (* Coverage error? *)

    let option g = 
        fmap (fun p -> if p < 2 then None else Some (g ())) (int_bound 10)
    ?$\vdash \Code{option}: \forall X{:}\kb.\forall p{:}(b\sarr\Bool). \Murt{b}{p(\vnu)}\sarr \Murt{(\Option[b])}{\vnu = \None \lor \exists x.p(x) \land \vnu = \Some[x]}$?

    let pair g1 g2 = fun () -> (g1 (), g2 ())
    ?$\vdash \Code{pair}: \forall X_1\;X_2{:}\kb.\forall p_1{:}(X_1\sarr\Bool)\;p_2{:}(X_2\sarr\Bool).$?
        ?$\Murt{X_1}{p_1(\vnu)}\sarr \Murt{X_2}{p_2(\vnu)}\sarr \Murt{X_1 \times X_2}{p_1(\fst(\vnu)) \land p_2(\snd(\vnu))}$?
\end{minted}

\begin{minted}[xleftmargin=5pt, numbersep=4pt, linenos = true, fontsize = \footnotesize, escapeinside=??]{OCaml}
    (* Others *)

    let oneofl l =
        return (List.nth l (Random.range 0 (List.length l)))
    ?$\vdash \Code{oneofl}: \forall X{:}\kb.\forall l{:}\List[X] \sarr \Murt{X}{\mem(l,\vnu)}$?

    let frequencyl (distr: int list) (l: 'b list) =
        let m = sum distr in
        let rec aux (acc: int) distr l =
            match (distr, l) with
            | ([], _) -> err
            | (n :: disr, x :: l) ->
                if m < acc+n then return x else aux (acc+n) ls
        in
        aux 0 distr l
    ?$\vdash \Code{frequencyl}: \forall X{:}\kb. d{:}\List[\Int] \sarr l{:}\ort{\List[X]}{\len(\vnu) = \len(d)} \sarr \Murt{b}{\mem(l,\vnu)}$?
    
    let numeral = 
        fmap (fun c -> char_of_int (c+48)) (int_bound 10)
    ?$\vdash \Code{numeral}: \Murt{\Char}{\I{numeral}(\vnu)}$?

    let list_size (size_gen: int -> unit) (gen: unit -> 'b) =
        let rec f (n: int) =
            if n <= 0 then [] else (gen ()) :: (f (n - 1))
        in fmap f size_gen
    ?$\vdash \Code{list\_size}: \forall X{:}\kb.\forall p_1{:}(\Int\sarr\Bool)\;p_2{:}(b\sarr\Bool).$?
        ?$\Murt{int}{p_1(\vnu)}\sarr \Murt{b}{p_2(\vnu)} \sarr \Murt{\List[X]}{p_1(len(\vnu)) \land \forall (x{:}b). \mem(\vnu, x) \impl p_2(x)}$?

    let list_repeat (n: int) (gen: unit -> 'b) = list_size (return n) gen
    ?$\vdash \Code{list\_repeat}: \forall X{:}\kb.\forall p{:}(b\sarr\Bool).$?
        ?$n{:}\ort{\Int}{0 \leq \vnu}\sarr \Murt{b}{p_2(\vnu)} \sarr \Murt{\List[X]}{len(\vnu) = n \land \forall (x{:}b). \mem(\vnu, x) \impl p_2(x)}$?
    
    (* A little bit worry about EPR constraint. *)

    let shuffle_l l = 
        let rec aux (i: int) (l: 'b list) =
            if i == 0 then l else
                aux (i - 1) (swap l (int_range 0 i ()) i)
        in
        fun () -> aux (List.length l - 1) l
    ?$\vdash \Code{shuffle\_l}: l{:}\List[\Int] \sarr \Murt{\List[\Int]}{\I{include}(\vnu, l)}$?

    let range_subset size low high st =
        let range_size = high - low + 1 in
        if not (0 <= size && size <= range_size) then err
        (* Floyd–Rivest algorithm *)
        let rec mk_set (i: int) (idxs: int list) =
            if i >= range_size then s
            else
                let pos = int_bound i () in
                let (choice: int) = if List.mem pos idxs then i else pos in
                mk_set (i+1) (choice :: idxs)
        in
        mk_set (range_size - size) []
    ?$\vdash \Code{list\_size}: \Code{size}{:}\Int \sarr \Code{low}{:}\Int \sarr \Code{high}{:}\ort{int}{\Code{low + size} < \vnu} \sarr$?
        ?$\Murt{\List[\Int]}{\uniq(\vnu) \land \minP(\vnu) = \Code{low} \land \maxP(\vnu) = \Code{high}}$?

    let pos_split2 n = 
        if (n < 2) then err else
            fmap (fun n1 -> (n1, n - n1)) (int_range 1 (n - 1))
    ?$\vdash \Code{list\_size}: n{:}\ort{\Int}{2 \leq n} \sarr$?
        ?$\Murt{(\Int\times\Int)}{\fst(\vnu) + \snd(\vnu) = n \land \fst(\vnu) > 0 \land \snd(\vnu) > 0}$?
\end{minted}

\paragraph{EPR} There is actually an invariant we keep during the type check, which is the under binding (i.e., $x{:}\urt{b}{\phi}$) can only be refer by the left-hand-side type of subtyping (the $\tau1$ in $\Gamma \vdash \tau_1 <: \tau_2$) because the $\tau_2$. Note that we disallow under parameter, thus all under types in type context comes from the local variables, which is hidden for the right-hand-side type (the checking type in bidirectional typing). In other world, we can use $\Code{exists}$ function to merge all under types in the type context into the left-hand-side type (synthesized type). Then, the subtyping is actually in the following format:
\begin{align*}
    \overline{x{:}\ort{b_x}{\phi_x}} \vdash \urt{b}{\overline{\exists y}.\phi_1} <: \urt{b}{\phi_2}
\end{align*}\noindent
which leads the following verification condition:
\begin{align*}
    \overline{\forall X{:}\kb}.\phi_x \impl \forall v.\phi_2 \impl \overline{\exists y}.\phi_1
\end{align*}\noindent
Then, $\phi_x$ can only be $\exists\phi$, $\phi_2$ can be $\exists\forall\phi$, and $\phi_1$ can only be $\exists\phi$. In general, most of qualifiers are just $\exists\phi$, which is also the constraint I suggest.


==> sections/changes.tex <==
\newpage
\section{Summary of Revisions}

We have attached three files: (a) poirot.pdf is the revised version of the paper, (b) poirot-diff.pdf highlights the text corresponding to major changes in \textcolor{CBLightOrange}{orange} (typo fixes and minor edits are not highlighted), and (c) poirot-sm.pdf contains our supplementary material.

The major changes are:
\begin{enumerate}
    \item We have added an additional case study in Section 6.2 (line $905$ - $957$), which describes the verification of a generator for well-typed STLC terms (Reviewer-D). This section provides a detailed description of the evaluation setting and results, and includes a discussion of the user effort needed by Poirot.
    \item We have added a completeness theorem for our bidirectional typing algorithm (Theorem 5.4 on lines $821$ - $824$) in Section 5. The corresponding proof is included in our supplemental material (Reviewer-B).
    \item We have explained the limitation of our tool on line $828$ (Reviewer-A).
    \item We have included the suggested related works on line $1022$ - $1025$ in Section 7 (Reviewer-B).
    \item We have revised the example in the overview so that commented code in Figure 1 is on a standalone line (Reviewer-B).
    \item We have integrated comments on the relationship to Incorrectness Logic to Sections 1 and 2 (line $132$, $134$ - $138$, $199$ - $200$, and $292$ - $293$) to help readers understand these connections earlier (Reviewer-A).
    \item We have clarified that our refinement typing rules assume that all terms are well-typed according to the normal (i.e. non-refined) type system on lines $484$ - $485$ (Reviewer-C).
    \item We now include related work on the distribution of data and fairness on lines $1054$ - $1061$ in Section (Reviewer-C).
    \item We have added a comment about the feasibility of enumerating data on $45$ - $46$ in the introduction (Reviewer-D).
    \item We have clarified the type context (line $302$ and $319$) and the explanation of coverage type (line $322$- $323$) in the last example in the overview (Reviewer-C).
    \item We have rephrased our discussion of reasoning about coverage (line $121$ - $130$) in the introduction.
    \item We have added a footnote on line $438$ - $439$ pointing to the full set of definitions included in the supplementary material.
    \item We now include a new column in Table 1 to indicate if the test input generator is recursive (previously we use the notation $\dagger$).
\end{enumerate}


==> sections/cover_letter.tex <==
%Abstract for submission

Test input generators are an important part of property-based testing (PBT) frameworks. Because PBT is intended to test deep semantic and structural properties of a program, the outputs produced by these generators can be complex data structures, constrained to satisfy properties the developer believes is most relevant to testing the function of interest. An important feature expected of these generators is that they be capable of producing <i>all</i> acceptable elements that satisfy the function's input type and generator-provided constraints. However, it is not readily apparent how we might validate whether a particular generator's output satisfies this <i>coverage</i> requirement. Typically, developers must rely on manual inspection and post-mortem analysis of test runs to determine if the generator is providing sufficient coverage; these approaches are error-prone and difficult to scale as generators become more complex. To address this important concern, we present a new refinement type-based verification procedure for validating the coverage provided by input test generators, based on a novel interpretation of types that embeds "<i>must</i>-style" underapproximate reasoning principles as a fundamental part of the type system. The types associated with expressions now capture the set of values <i>guaranteed</i> to be produced by the expression, rather than the typical formulation that uses types to represent the set of values an expression <i>may</i> produce. We have formalized the notion of <i>coverage types</i> in a rich core language that supports higher-order functions and inductive datatype; to better support checking coverage properties of real-world test generators, we extend this type system with type and qualifier polymorphism. These extensions enable our system to statically verify coverage guarantees of test input generators constructed using the the sort of monadic combinators provided by most PBT frameworks. We have implemented a coverage type checker for OCaml programs based on this core calculus, and present a detailed evaluation of the utility of our ideas using a corpus of benchmarks drawn from both the PBT literature and open source projects.

% cover letter

Dear Editor,

We are pleased to submit our manuscript <i>Polymorphic Coverage Types</i>. This submission is an extended version of our PLDI 2023 conference paper. We have included the following files for your review:
(a) <b>poirot-jfp.pdf</b> – the main article,
(b) <b>poirot-jfp-diff.pdf</b> – a marked-up version highlighting major changes in blue (minor edits are not highlighted), and
(c) <b>poirot-jfp-sm.pdf</b> – the supplementary material.

While we have augmented the material from the PLDI 2023 version of the paper with additional details and examples, the bulk of the new material consists of a polymorphic extension to the previous type system (Section 7), which we use to define a novel coverage monad and to type check a collection of generator combinators inspired by OCaml's QCheck PBT framework (Section 8). We have also extended the previous evaluation with a substantial new case study (Section 9) that uses these new features to check coverage properties of a set of real-world input generators drawn from open-source projects that use PBT.

==> sections/cover_letter2.tex <==
Dear Editor,

We appreciate the reviewers' detailed feedback and suggestions.
In response, we have made the following revisions to our manuscript:
\begin{itemize}
    \item We have clarified our data availability statement in Section 12, and specified that the mechanized proof is about our soundness theorem (Theorem~5.3). (Reviewers 1 and 3)
    \item We have added a discussion at the end of Section 9 (line 2080 - 2127) highlighting the practical benefits our type system offers to test engineers. (Reviewer 2)
    \item We have provided further details and clarifications regarding our subtyping rules in Section 4 (line 589 - 608, line 641 - 692). (Reviewer 1)
    \item Throughout the paper, we now use the term ``method predicate'' in place of ``uninterpreted predicate.'' (Reviewer 2)
    \item We have corrected all typos identified by the reviewers.
\end{itemize}

We have included the following files for your review:
(a) <b>poirot-jfp.pdf</b> - the main article,
(b) <b>poirot-jfp-diff.pdf</b> - a marked-up version highlighting major changes in blue (minor edits are not highlighted), and
(c) <b>poirot-jfp-sm.pdf</b> - the supplementary material.



==> sections/news.tex <==
\section{Random}

Mutable random state, force persistence.
\begin{align*}
    &\Gamma \vdash \mathcal{r} \typeinfer [\mathcal{r}] \\
    &\Gamma \vdash \S{gen} \typeinfer [\mathcal{r}] \to \nuut{int}{\top} \quad \text{built-in operator like $+$}
\end{align*}

\begin{lstlisting}[language = ocaml,linewidth=330pt, xleftmargin=50pt, frame=none]
let nat_gen (r: random_state) =
  let (x: int) = gen r in
  if x < 0 then Exn else x
\end{lstlisting}

Or, immutable random state, treat is normally.
\begin{align*}
    &\Gamma \vdash \mathcal{r} \typeinfer \nuut{t}{\top} \\
    &\Gamma \vdash \S{gen} \typeinfer \nuut{t}{\top} \to (\nuut{t}{\top} \times \nuut{int}{\top}) 
\end{align*}

\begin{lstlisting}[language = ocaml,linewidth=330pt, xleftmargin=50pt, frame=none]
let rec nat_gen (r: random_state) =
    let (r: random_state), (x: int) = gen r in
    if x < 0 then nat_gen r else x
\end{lstlisting}

\section{Ranking Function}

\begin{lstlisting}[language = ocaml,linewidth=430pt, xleftmargin=50pt, frame=none]
let rec list_gen ((size : int) [@rankfunc? n when size]) (x : int) =
  if size == 0 then []
  else
    let (size2 : int) = size - 1 in
    let (l : int list) = list_gen size2 x in
    let (l2 : int list) = x :: l in
    l2
\end{lstlisting}
Should have type:
\begin{align*}
    \nuutarr{size}{int}{\nu \leq 0} \nuutarr{x}{int}{\nu = ?} \nuut{int\ list}{\forall u, \mem{\nu}{u} \impl u = x}
\end{align*}

Should have type:
\begin{align*}
    \nuutarr{size}{int}{\nu \leq 0} \xarr{x}{int} \nuut{int\ list}{\forall u, \mem{\nu}{u} \impl u = x}
\end{align*}

Should have type:
\begin{align*}
    \xarr{size}{int} \xarr{x}{int} \nuut{int\ list}{\I{len}(\nu, size) \land \forall u, \mem{\nu}{u} \impl u = x}
\end{align*}


Typing rule:

\begin{prooftree}
\hypo{
\parbox{130mm}{\raggedright
$\forall n, n = 0 \implies f{:}\nuut{t}{\bot}\ x{:}(\tau_x \land \nuut{int}{rank(\nu) = n}) \vdash e \typecheck \tau$ \\
$\forall n, n > 0 \implies f{:}x{:}(\tau_x \land \nuut{int}{rank(\nu) < n}) \to \tau\ x{:}(\tau_x \land \nuut{int}{ rank(\nu) = n}) \vdash e \typecheck \tau $
}} 
\infer1[Check-Infer]{ 
\Gamma \vdash (\S{fix}\ f\ \lambda x. e) \typecheck x{:}\tau_x{|}\langle n \equiv rank(x) \rangle \to \tau
}
\end{prooftree}

\begin{align*}
    &\forall n, n = 0 \implies \\
    &\S{list\_gen}{:}\xarr{size}{int} \xarr{x}{int} \nuut{t}{\bot} \\
    & \hat{size}{:}\nuut{int}{\top \land \nu = n}\ \hat{x}{:}\nuut{int}{\top}\  \vdash e \typecheck
    \nuut{int\ list}{\I{len}(\nu, size) \land \forall u, \mem{\nu}{u} \impl u = x}
\end{align*}

\begin{align*}
    &\forall n, n > 0 \implies \\
    &\S{list\_gen}{:}\nuutarr{\hat{size}}{int}{\nu < n} \xarr{x}{int}  \nuut{int\ list}{\I{len}(\nu, size) \land \forall u, \mem{\nu}{u} \impl u = x} \\
    & \hat{size}{:}\nuut{int}{\top \land \nu = n}\ \hat{x}{:}\nuut{int}{\top}\  \vdash e \typecheck
    \nuut{int\ list}{\I{len}(\nu, size) \land \forall u, \mem{\nu}{u} \impl u = x}
\end{align*}
